Applying the Gricean Maxims to a Human-LLM Interaction Cycle: Design Insights from a Participatory Approach

While large language models (LLMs) are increasingly used to assist users in various tasks through natural language interactions, these interactions often fall short due to LLMs' limited ability to infer contextual nuances and user intentions, unlike humans. To address this challenge, we draw inspiration from the Gricean Maxims--human communication theory that suggests principles of effective communication--and aim to derive design insights for enhancing human-AI interactions (HAI). Through participatory design workshops with communication experts, designers, and end-users, we identified ways to apply these maxims across the stages of the HAI cycle. Our findings include reinterpreted maxims tailored to human-LLM contexts and nine actionable design considerations categorized by interaction stage. These insights provide a concrete framework for designing more cooperative and user-centered LLM-based systems, bridging theoretical foundations in communication with practical applications in HAI.

==> tables/redefinition.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|l|l}
\toprule
\textbf{Gricean Maxims} & \textbf{Original Definition} & \textbf{Redefining Gricean Maxims in the Context of Human-LLM Interaction} \\ 
\midrule
\textbf{Quantity} & \begin{tabular}[c]{@{}l@{}}Make your contribution as informative as is required \\ (for the current purposes of the exchange).\\ Do not make your contribution more informative than is required.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Not only to provide the right amount of information but also to present it \\in a way that optimizes the user's cognitive load, allowing them to navigate \\ and explore the depth and amount of information hierarchically based on their needs.\end{tabular} \\ \hline
\textbf{Quality} & \begin{tabular}[c]{@{}l@{}}Do not say what you believe is false.\\ Do not say that for which you lack adequate evidence.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Beyond simply providing truthful and reliable information, \\ this maxim includes fostering the user's trust in the LLM. \\ This encompasses ensuring that the user perceives the LLM \\ as a trustworthy and efficient partner capable of aiding their tasks.\end{tabular} \\ \hline
\textbf{Relation} &  \begin{tabular}[c]{@{}l@{}} The information provided should be relevant to the \\ current exchange and omit any irrelevant information. \end{tabular} & \begin{tabular}[c]{@{}l@{}}In human-LLM interactions, relevance goes beyond just responding to the \\ immediate query at hand. The LLM needs to comprehend the broader context, \\ including the user's goals and intentions behind their tasks. %, while also maintaining \\ the flow of the conversation and acting in a manner that remains \\ relevant throughout the entire interaction.
\end{tabular} \\ \hline
\textbf{Manner} & \begin{tabular}[c]{@{}l@{}}Avoid obscurity of expression.\\ Avoid ambiguity.\\ Be brief.\\ Be orderly.\end{tabular} & \begin{tabular}[c]{@{}l@{}} Beyond avoiding ambiguity and being brief and orderly, this maxim includes that \\ the LLM should adapt its response format to suit the user’s requirements \\ —whether through bullet points, summaries, detailed explanations, or code.\end{tabular} \\ 
\bottomrule
\end{tabular}%
}
\caption{Redefinition of Gricean Maxims in the human-LLM interaction context.}
\label{tab:redefinition}
\end{table}
